Graph Clustering with Graph Neural Networks

Graph Neural Networks (GNNs) have achieved state-of-the-art results on many graph analysis tasks such as node classification and link prediction. However, important unsupervised problems on graphs, such as graph clustering, have proved more resistant to advances in GNNs. Graph clustering has the same overall goal as node pooling in GNNs - does this mean that GNN pooling methods do a good job at clustering graphs? Surprisingly, the answer is no - current GNN pooling methods often fail to recover the cluster structure in cases where simple baselines, such as k-means applied on learned representations, work well. We investigate further by carefully designing a set of experiments to study different signal-to-noise scenarios both in graph structure and attribute data. To address these methods' poor performance in clustering, we introduce Deep Modularity Networks (DMoN), an unsupervised pooling method inspired by the modularity measure of clustering quality, and show how it tackles recovery of the challenging clustering structure of real-world graphs. Similarly, on real-world data, we show that DMoN produces high quality clusters which correlate strongly with ground truth labels, achieving state-of-the-art results with over 40% improvement over other pooling methods across different metrics.

==> data/loss_histories.tex <==
epoch mgcn mgcn-reg mincut mincut-reg
0 -0.0158 0.0001 -0.9972 1.2227
1 -0.0158 0.0000 -0.9975 1.2227
2 -0.0159 0.0001 -0.9977 1.2226
3 -0.0160 0.0001 -0.9980 1.2224
4 -0.0161 0.0001 -0.9979 1.2220
5 -0.0162 0.0000 -0.9976 1.2215
6 -0.0164 0.0000 -0.9974 1.2207
7 -0.0167 0.0000 -0.9971 1.2195
8 -0.0171 0.0001 -0.9965 1.2178
9 -0.0177 0.0001 -0.9956 1.2155
10 -0.0185 0.0002 -0.9944 1.2120
11 -0.0197 0.0004 -0.9928 1.2071
12 -0.0215 0.0007 -0.9907 1.2002
13 -0.0241 0.0013 -0.9880 1.1906
14 -0.0277 0.0021 -0.9849 1.1781
15 -0.0327 0.0033 -0.9816 1.1627
16 -0.0393 0.0051 -0.9784 1.1450
17 -0.0478 0.0074 -0.9754 1.1255
18 -0.0582 0.0103 -0.9728 1.1041
19 -0.0703 0.0138 -0.9703 1.0813
20 -0.0840 0.0178 -0.9681 1.0580
21 -0.0989 0.0222 -0.9666 1.0351
22 -0.1148 0.0271 -0.9656 1.0127
23 -0.1317 0.0323 -0.9650 0.9912
24 -0.1493 0.0379 -0.9647 0.9703
25 -0.1672 0.0436 -0.9644 0.9500
26 -0.1850 0.0493 -0.9639 0.9299
27 -0.2022 0.0543 -0.9631 0.9098
28 -0.2184 0.0584 -0.9619 0.8894
29 -0.2336 0.0613 -0.9603 0.8691
30 -0.2477 0.0630 -0.9588 0.8490
31 -0.2611 0.0637 -0.9576 0.8292
32 -0.2739 0.0638 -0.9565 0.8090
33 -0.2860 0.0636 -0.9552 0.7890
34 -0.2973 0.0634 -0.9538 0.7704
35 -0.3076 0.0631 -0.9526 0.7527
36 -0.3169 0.0629 -0.9516 0.7346
37 -0.3256 0.0626 -0.9504 0.7161
38 -0.3334 0.0622 -0.9489 0.6974
39 -0.3406 0.0618 -0.9471 0.6784
40 -0.3471 0.0613 -0.9453 0.6587
41 -0.3527 0.0609 -0.9435 0.6377
42 -0.3577 0.0606 -0.9418 0.6149
43 -0.3621 0.0603 -0.9402 0.5900
44 -0.3659 0.0601 -0.9387 0.5627
45 -0.3693 0.0600 -0.9372 0.5334
46 -0.3723 0.0600 -0.9358 0.5026
47 -0.3751 0.0600 -0.9344 0.4709
48 -0.3778 0.0601 -0.9330 0.4394
49 -0.3802 0.0602 -0.9314 0.4087
50 -0.3825 0.0603 -0.9296 0.3784
51 -0.3847 0.0604 -0.9278 0.3490
52 -0.3866 0.0605 -0.9261 0.3232
53 -0.3884 0.0606 -0.9251 0.2993
54 -0.3900 0.0607 -0.9243 0.2753
55 -0.3914 0.0608 -0.9232 0.2540
56 -0.3928 0.0609 -0.9223 0.2340
57 -0.3940 0.0609 -0.9215 0.2155
58 -0.3950 0.0610 -0.9207 0.1997
59 -0.3960 0.0610 -0.9200 0.1846
60 -0.3969 0.0610 -0.9192 0.1707
61 -0.3977 0.0611 -0.9184 0.1588
62 -0.3984 0.0611 -0.9177 0.1481
63 -0.3991 0.0611 -0.9170 0.1388
64 -0.3997 0.0612 -0.9165 0.1309
65 -0.4002 0.0612 -0.9161 0.1239
66 -0.4007 0.0612 -0.9160 0.1175
67 -0.4012 0.0612 -0.9161 0.1118
68 -0.4016 0.0612 -0.9163 0.1066
69 -0.4020 0.0612 -0.9165 0.1022
70 -0.4024 0.0612 -0.9169 0.0986
71 -0.4028 0.0612 -0.9173 0.0954
72 -0.4031 0.0612 -0.9175 0.0922
73 -0.4034 0.0612 -0.9176 0.0888
74 -0.4037 0.0612 -0.9175 0.0853
75 -0.4040 0.0612 -0.9175 0.0819
76 -0.4042 0.0612 -0.9174 0.0790
77 -0.4044 0.0612 -0.9173 0.0766
78 -0.4046 0.0612 -0.9172 0.0742
79 -0.4048 0.0612 -0.9172 0.0720
80 -0.4050 0.0612 -0.9172 0.0699
81 -0.4052 0.0612 -0.9173 0.0680
82 -0.4053 0.0612 -0.9175 0.0662
83 -0.4055 0.0612 -0.9177 0.0645
84 -0.4056 0.0612 -0.9179 0.0629
85 -0.4058 0.0613 -0.9181 0.0612
86 -0.4059 0.0613 -0.9182 0.0596
87 -0.4060 0.0613 -0.9183 0.0582
88 -0.4061 0.0613 -0.9184 0.0569
89 -0.4062 0.0613 -0.9184 0.0556
90 -0.4063 0.0613 -0.9185 0.0543
91 -0.4064 0.0613 -0.9186 0.0530
92 -0.4065 0.0613 -0.9188 0.0518
93 -0.4066 0.0613 -0.9189 0.0506
94 -0.4067 0.0613 -0.9190 0.0494
95 -0.4068 0.0613 -0.9191 0.0483
96 -0.4068 0.0613 -0.9192 0.0473
97 -0.4069 0.0613 -0.9193 0.0463
98 -0.4070 0.0613 -0.9193 0.0453
99 -0.4070 0.0613 -0.9194 0.0444
100 -0.4071 0.0613 -0.9195 0.0435
101 -0.4071 0.0613 -0.9196 0.0427
102 -0.4072 0.0613 -0.9197 0.0420
103 -0.4072 0.0613 -0.9198 0.0413
104 -0.4073 0.0613 -0.9199 0.0406
105 -0.4073 0.0613 -0.9200 0.0399
106 -0.4074 0.0613 -0.9201 0.0393
107 -0.4074 0.0613 -0.9202 0.0387
108 -0.4075 0.0613 -0.9203 0.0381
109 -0.4075 0.0613 -0.9204 0.0375
110 -0.4076 0.0613 -0.9205 0.0370
111 -0.4076 0.0613 -0.9206 0.0365
112 -0.4077 0.0613 -0.9207 0.0360
113 -0.4077 0.0613 -0.9208 0.0355
114 -0.4077 0.0613 -0.9209 0.0350
115 -0.4078 0.0613 -0.9210 0.0345
116 -0.4078 0.0613 -0.9211 0.0340
117 -0.4078 0.0613 -0.9212 0.0336
118 -0.4079 0.0613 -0.9213 0.0332
119 -0.4079 0.0613 -0.9214 0.0328
120 -0.4079 0.0613 -0.9215 0.0324
121 -0.4080 0.0613 -0.9216 0.0320
122 -0.4080 0.0613 -0.9217 0.0317
123 -0.4080 0.0613 -0.9218 0.0313
124 -0.4080 0.0613 -0.9219 0.0310
125 -0.4081 0.0613 -0.9219 0.0307
126 -0.4081 0.0613 -0.9220 0.0303
127 -0.4081 0.0613 -0.9221 0.0300
128 -0.4081 0.0613 -0.9221 0.0298
129 -0.4082 0.0613 -0.9222 0.0295
130 -0.4082 0.0613 -0.9223 0.0292
131 -0.4082 0.0613 -0.9223 0.0289
132 -0.4082 0.0613 -0.9223 0.0286
133 -0.4082 0.0613 -0.9224 0.0284
134 -0.4083 0.0613 -0.9224 0.0281
135 -0.4083 0.0613 -0.9224 0.0279
136 -0.4083 0.0613 -0.9225 0.0277
137 -0.4083 0.0612 -0.9225 0.0274
138 -0.4084 0.0612 -0.9225 0.0272
139 -0.4084 0.0612 -0.9225 0.0270
140 -0.4084 0.0612 -0.9225 0.0268
141 -0.4084 0.0612 -0.9225 0.0266
142 -0.4084 0.0612 -0.9225 0.0264
143 -0.4085 0.0612 -0.9226 0.0262
144 -0.4085 0.0612 -0.9226 0.0260
145 -0.4085 0.0612 -0.9226 0.0258
146 -0.4086 0.0612 -0.9227 0.0256
147 -0.4086 0.0612 -0.9227 0.0255
148 -0.4086 0.0612 -0.9227 0.0253
149 -0.4087 0.0612 -0.9228 0.0251
150 -0.4087 0.0611 -0.9228 0.0250
151 -0.4088 0.0611 -0.9228 0.0248
152 -0.4088 0.0611 -0.9229 0.0247
153 -0.4088 0.0611 -0.9229 0.0246
154 -0.4089 0.0611 -0.9229 0.0244
155 -0.4089 0.0611 -0.9229 0.0243
156 -0.4089 0.0611 -0.9230 0.0241
157 -0.4089 0.0611 -0.9230 0.0240
158 -0.4089 0.0611 -0.9230 0.0239
159 -0.4090 0.0611 -0.9230 0.0237
160 -0.4090 0.0611 -0.9231 0.0236
161 -0.4090 0.0611 -0.9231 0.0235
162 -0.4090 0.0611 -0.9231 0.0234
163 -0.4090 0.0611 -0.9231 0.0232
164 -0.4091 0.0611 -0.9232 0.0231
165 -0.4091 0.0611 -0.9232 0.0230
166 -0.4091 0.0611 -0.9232 0.0228
167 -0.4091 0.0611 -0.9232 0.0227
168 -0.4091 0.0611 -0.9233 0.0226
169 -0.4091 0.0611 -0.9233 0.0224
170 -0.4092 0.0611 -0.9233 0.0223
171 -0.4092 0.0611 -0.9234 0.0222
172 -0.4092 0.0611 -0.9234 0.0221
173 -0.4092 0.0611 -0.9234 0.0219
174 -0.4092 0.0611 -0.9234 0.0218
175 -0.4092 0.0611 -0.9235 0.0217
176 -0.4092 0.0611 -0.9235 0.0215
177 -0.4093 0.0611 -0.9235 0.0214
178 -0.4093 0.0611 -0.9235 0.0213
179 -0.4093 0.0611 -0.9235 0.0211
180 -0.4093 0.0611 -0.9235 0.0210
181 -0.4093 0.0611 -0.9236 0.0209
182 -0.4093 0.0611 -0.9236 0.0207
183 -0.4093 0.0611 -0.9236 0.0206
184 -0.4093 0.0611 -0.9236 0.0205
185 -0.4093 0.0611 -0.9236 0.0204
186 -0.4094 0.0611 -0.9236 0.0203
187 -0.4094 0.0611 -0.9237 0.0202
188 -0.4094 0.0611 -0.9237 0.0201
189 -0.4094 0.0611 -0.9237 0.0200
190 -0.4094 0.0611 -0.9237 0.0199
191 -0.4094 0.0611 -0.9237 0.0198
192 -0.4094 0.0611 -0.9238 0.0197
193 -0.4094 0.0612 -0.9238 0.0196
194 -0.4094 0.0612 -0.9238 0.0195
195 -0.4094 0.0612 -0.9238 0.0194
196 -0.4095 0.0612 -0.9238 0.0193
197 -0.4095 0.0612 -0.9239 0.0192
198 -0.4095 0.0612 -0.9239 0.0191
199 -0.4095 0.0612 -0.9239 0.0190
200 -0.4095 0.0612 -0.9239 0.0189
201 -0.4095 0.0612 -0.9239 0.0188
202 -0.4095 0.0612 -0.9239 0.0188
203 -0.4095 0.0612 -0.9240 0.0187
204 -0.4095 0.0612 -0.9240 0.0186
205 -0.4095 0.0612 -0.9240 0.0186
206 -0.4095 0.0612 -0.9240 0.0185
207 -0.4095 0.0612 -0.9240 0.0184
208 -0.4095 0.0612 -0.9240 0.0184
209 -0.4095 0.0612 -0.9241 0.0183
210 -0.4096 0.0612 -0.9241 0.0183
211 -0.4096 0.0612 -0.9241 0.0182
212 -0.4096 0.0612 -0.9241 0.0181
213 -0.4096 0.0612 -0.9241 0.0181
214 -0.4096 0.0612 -0.9241 0.0180
215 -0.4096 0.0612 -0.9242 0.0180
216 -0.4096 0.0612 -0.9242 0.0179
217 -0.4096 0.0612 -0.9242 0.0179
218 -0.4096 0.0612 -0.9242 0.0178
219 -0.4096 0.0612 -0.9242 0.0178
220 -0.4096 0.0612 -0.9243 0.0177
221 -0.4096 0.0612 -0.9243 0.0177
222 -0.4096 0.0612 -0.9243 0.0176
223 -0.4096 0.0612 -0.9243 0.0176
224 -0.4097 0.0612 -0.9244 0.0175
225 -0.4097 0.0612 -0.9244 0.0174
226 -0.4097 0.0611 -0.9244 0.0174
227 -0.4098 0.0611 -0.9244 0.0173
228 -0.4098 0.0611 -0.9244 0.0173
229 -0.4099 0.0611 -0.9244 0.0172
230 -0.4100 0.0611 -0.9245 0.0172
231 -0.4100 0.0611 -0.9245 0.0171
232 -0.4100 0.0611 -0.9245 0.0171
233 -0.4100 0.0611 -0.9245 0.0171
234 -0.4100 0.0611 -0.9245 0.0170
235 -0.4100 0.0611 -0.9245 0.0170
236 -0.4100 0.0611 -0.9245 0.0169
237 -0.4100 0.0611 -0.9245 0.0169
238 -0.4101 0.0611 -0.9246 0.0169
239 -0.4101 0.0611 -0.9246 0.0168
240 -0.4101 0.0611 -0.9246 0.0168
241 -0.4101 0.0611 -0.9246 0.0168
242 -0.4101 0.0611 -0.9246 0.0167
243 -0.4101 0.0611 -0.9246 0.0167
244 -0.4101 0.0612 -0.9246 0.0167
245 -0.4101 0.0612 -0.9246 0.0166
246 -0.4101 0.0612 -0.9246 0.0166
247 -0.4101 0.0612 -0.9246 0.0166
248 -0.4101 0.0612 -0.9246 0.0165
249 -0.4102 0.0612 -0.9247 0.0165
250 -0.4102 0.0612 -0.9247 0.0165
251 -0.4102 0.0612 -0.9247 0.0165
252 -0.4102 0.0612 -0.9247 0.0164
253 -0.4102 0.0612 -0.9247 0.0164
254 -0.4102 0.0612 -0.9247 0.0164
255 -0.4102 0.0612 -0.9247 0.0163
256 -0.4102 0.0612 -0.9247 0.0163
257 -0.4102 0.0612 -0.9247 0.0163
258 -0.4102 0.0612 -0.9247 0.0163
259 -0.4102 0.0612 -0.9247 0.0162
260 -0.4102 0.0612 -0.9247 0.0162
261 -0.4102 0.0612 -0.9247 0.0162
262 -0.4102 0.0612 -0.9247 0.0162
263 -0.4102 0.0612 -0.9247 0.0162
264 -0.4102 0.0612 -0.9247 0.0161
265 -0.4103 0.0612 -0.9247 0.0161
266 -0.4103 0.0612 -0.9247 0.0161
267 -0.4103 0.0612 -0.9248 0.0161
268 -0.4104 0.0612 -0.9248 0.0161
269 -0.4104 0.0612 -0.9248 0.0160
270 -0.4104 0.0612 -0.9248 0.0160
271 -0.4104 0.0612 -0.9248 0.0160
272 -0.4104 0.0612 -0.9248 0.0160
273 -0.4104 0.0612 -0.9248 0.0160
274 -0.4104 0.0612 -0.9249 0.0160
275 -0.4105 0.0612 -0.9249 0.0160
276 -0.4105 0.0612 -0.9249 0.0160
277 -0.4105 0.0612 -0.9249 0.0159
278 -0.4105 0.0612 -0.9250 0.0159
279 -0.4105 0.0611 -0.9250 0.0159
280 -0.4105 0.0611 -0.9250 0.0159
281 -0.4105 0.0611 -0.9250 0.0159
282 -0.4105 0.0611 -0.9251 0.0159
283 -0.4105 0.0611 -0.9251 0.0159
284 -0.4105 0.0611 -0.9251 0.0159
285 -0.4105 0.0611 -0.9251 0.0159
286 -0.4105 0.0611 -0.9252 0.0159
287 -0.4105 0.0611 -0.9252 0.0159
288 -0.4105 0.0611 -0.9252 0.0158
289 -0.4105 0.0611 -0.9252 0.0158
290 -0.4105 0.0611 -0.9252 0.0158
291 -0.4106 0.0611 -0.9253 0.0158
292 -0.4106 0.0611 -0.9253 0.0158
293 -0.4106 0.0611 -0.9253 0.0157
294 -0.4106 0.0611 -0.9253 0.0157
295 -0.4106 0.0611 -0.9253 0.0157
296 -0.4106 0.0611 -0.9253 0.0157
297 -0.4106 0.0611 -0.9253 0.0157
298 -0.4106 0.0611 -0.9253 0.0157
299 -0.4106 0.0611 -0.9253 0.0156
300 -0.4106 0.0611 -0.9254 0.0156
301 -0.4106 0.0611 -0.9254 0.0156
302 -0.4106 0.0611 -0.9254 0.0156
303 -0.4106 0.0611 -0.9254 0.0156
304 -0.4106 0.0611 -0.9254 0.0156
305 -0.4106 0.0611 -0.9254 0.0156
306 -0.4106 0.0611 -0.9254 0.0155
307 -0.4107 0.0611 -0.9254 0.0155
308 -0.4107 0.0611 -0.9254 0.0155
309 -0.4107 0.0611 -0.9255 0.0155
310 -0.4107 0.0611 -0.9255 0.0155
311 -0.4107 0.0611 -0.9255 0.0155
312 -0.4107 0.0611 -0.9255 0.0155
313 -0.4107 0.0611 -0.9255 0.0155
314 -0.4107 0.0611 -0.9255 0.0154
315 -0.4107 0.0611 -0.9255 0.0154
316 -0.4108 0.0611 -0.9255 0.0154
317 -0.4108 0.0611 -0.9256 0.0154
318 -0.4108 0.0611 -0.9256 0.0154
319 -0.4108 0.0611 -0.9256 0.0154
320 -0.4108 0.0611 -0.9256 0.0153
321 -0.4108 0.0611 -0.9256 0.0153
322 -0.4108 0.0610 -0.9256 0.0153
323 -0.4108 0.0610 -0.9256 0.0153
324 -0.4108 0.0610 -0.9256 0.0153
325 -0.4108 0.0610 -0.9256 0.0153
326 -0.4108 0.0610 -0.9256 0.0153
327 -0.4108 0.0610 -0.9256 0.0153
328 -0.4109 0.0610 -0.9256 0.0153
329 -0.4109 0.0610 -0.9256 0.0152
330 -0.4109 0.0610 -0.9256 0.0152
331 -0.4110 0.0609 -0.9256 0.0152
332 -0.4110 0.0609 -0.9257 0.0152
333 -0.4111 0.0609 -0.9257 0.0152
334 -0.4111 0.0609 -0.9257 0.0152
335 -0.4111 0.0608 -0.9257 0.0152
336 -0.4111 0.0608 -0.9257 0.0152
337 -0.4111 0.0608 -0.9257 0.0152
338 -0.4111 0.0608 -0.9257 0.0152
339 -0.4111 0.0608 -0.9257 0.0152
340 -0.4111 0.0608 -0.9257 0.0152
341 -0.4111 0.0608 -0.9257 0.0152
342 -0.4111 0.0608 -0.9257 0.0152
343 -0.4111 0.0608 -0.9257 0.0151
344 -0.4111 0.0608 -0.9257 0.0151
345 -0.4111 0.0607 -0.9257 0.0151
346 -0.4111 0.0607 -0.9258 0.0151
347 -0.4112 0.0607 -0.9258 0.0151
348 -0.4112 0.0607 -0.9258 0.0151
349 -0.4113 0.0606 -0.9258 0.0151
350 -0.4115 0.0606 -0.9258 0.0151
351 -0.4116 0.0606 -0.9258 0.0151
352 -0.4117 0.0605 -0.9258 0.0151
353 -0.4117 0.0605 -0.9258 0.0151
354 -0.4118 0.0604 -0.9258 0.0151
355 -0.4118 0.0604 -0.9258 0.0150
356 -0.4118 0.0604 -0.9258 0.0150
357 -0.4118 0.0603 -0.9258 0.0150
358 -0.4118 0.0603 -0.9258 0.0150
359 -0.4119 0.0603 -0.9258 0.0150
360 -0.4119 0.0603 -0.9258 0.0150
361 -0.4119 0.0603 -0.9258 0.0150
362 -0.4120 0.0603 -0.9258 0.0150
363 -0.4120 0.0604 -0.9258 0.0150
364 -0.4120 0.0604 -0.9258 0.0150
365 -0.4121 0.0604 -0.9258 0.0150
366 -0.4121 0.0604 -0.9259 0.0150
367 -0.4121 0.0604 -0.9259 0.0149
368 -0.4121 0.0604 -0.9259 0.0149
369 -0.4121 0.0604 -0.9259 0.0149
370 -0.4122 0.0604 -0.9259 0.0149
371 -0.4122 0.0604 -0.9259 0.0149
372 -0.4122 0.0604 -0.9259 0.0149
373 -0.4122 0.0604 -0.9259 0.0149
374 -0.4122 0.0604 -0.9259 0.0149
375 -0.4122 0.0604 -0.9259 0.0149
376 -0.4122 0.0604 -0.9259 0.0149
377 -0.4122 0.0604 -0.9259 0.0149
378 -0.4122 0.0604 -0.9259 0.0149
379 -0.4122 0.0604 -0.9259 0.0149
380 -0.4122 0.0604 -0.9259 0.0148
381 -0.4122 0.0604 -0.9260 0.0148
382 -0.4122 0.0604 -0.9260 0.0148
383 -0.4122 0.0604 -0.9260 0.0148
384 -0.4122 0.0604 -0.9260 0.0148
385 -0.4122 0.0604 -0.9260 0.0148
386 -0.4122 0.0604 -0.9260 0.0148
387 -0.4122 0.0604 -0.9260 0.0148
388 -0.4122 0.0604 -0.9260 0.0147
389 -0.4122 0.0604 -0.9260 0.0147
390 -0.4122 0.0604 -0.9260 0.0147
391 -0.4122 0.0604 -0.9260 0.0147
392 -0.4122 0.0604 -0.9260 0.0147
393 -0.4122 0.0604 -0.9260 0.0147
394 -0.4122 0.0604 -0.9260 0.0147
395 -0.4122 0.0604 -0.9260 0.0147
396 -0.4123 0.0604 -0.9260 0.0146
397 -0.4123 0.0604 -0.9260 0.0146
398 -0.4123 0.0604 -0.9260 0.0146
399 -0.4123 0.0604 -0.9260 0.0146
400 -0.4123 0.0604 -0.9260 0.0146
401 -0.4123 0.0604 -0.9260 0.0146
402 -0.4123 0.0604 -0.9260 0.0146
403 -0.4123 0.0604 -0.9260 0.0146
404 -0.4123 0.0604 -0.9260 0.0145
405 -0.4123 0.0604 -0.9260 0.0145
406 -0.4123 0.0604 -0.9260 0.0145
407 -0.4123 0.0604 -0.9260 0.0145
408 -0.4123 0.0604 -0.9260 0.0145
409 -0.4123 0.0604 -0.9260 0.0145
410 -0.4123 0.0604 -0.9260 0.0145
411 -0.4123 0.0604 -0.9260 0.0145
412 -0.4123 0.0604 -0.9260 0.0144
413 -0.4123 0.0604 -0.9260 0.0144
414 -0.4123 0.0604 -0.9260 0.0144
415 -0.4123 0.0604 -0.9260 0.0144
416 -0.4123 0.0604 -0.9260 0.0144
417 -0.4123 0.0604 -0.9260 0.0144
418 -0.4123 0.0604 -0.9260 0.0144
419 -0.4123 0.0604 -0.9260 0.0144
420 -0.4123 0.0604 -0.9260 0.0143
421 -0.4123 0.0604 -0.9260 0.0143
422 -0.4123 0.0604 -0.9260 0.0143
423 -0.4123 0.0604 -0.9260 0.0143
424 -0.4123 0.0604 -0.9260 0.0143
425 -0.4123 0.0604 -0.9260 0.0143
426 -0.4123 0.0604 -0.9260 0.0143
427 -0.4123 0.0604 -0.9260 0.0142
428 -0.4123 0.0604 -0.9260 0.0142
429 -0.4123 0.0604 -0.9260 0.0142
430 -0.4123 0.0604 -0.9259 0.0142
431 -0.4123 0.0604 -0.9259 0.0142
432 -0.4123 0.0604 -0.9259 0.0142
433 -0.4123 0.0604 -0.9259 0.0142
434 -0.4123 0.0604 -0.9259 0.0142
435 -0.4123 0.0604 -0.9259 0.0142
436 -0.4123 0.0604 -0.9259 0.0141
437 -0.4123 0.0604 -0.9259 0.0141
438 -0.4123 0.0604 -0.9259 0.0141
439 -0.4123 0.0604 -0.9259 0.0141
440 -0.4123 0.0604 -0.9259 0.0141
441 -0.4123 0.0604 -0.9259 0.0141
442 -0.4123 0.0604 -0.9259 0.0141
443 -0.4123 0.0604 -0.9260 0.0141
444 -0.4123 0.0604 -0.9260 0.0141
445 -0.4123 0.0604 -0.9260 0.0141
446 -0.4124 0.0604 -0.9260 0.0141
447 -0.4124 0.0604 -0.9260 0.0141
448 -0.4124 0.0604 -0.9260 0.0141
449 -0.4124 0.0604 -0.9260 0.0141
450 -0.4124 0.0604 -0.9260 0.0141
451 -0.4124 0.0604 -0.9260 0.0140
452 -0.4124 0.0604 -0.9260 0.0140
453 -0.4124 0.0604 -0.9260 0.0140
454 -0.4124 0.0604 -0.9260 0.0140
455 -0.4124 0.0604 -0.9260 0.0140
456 -0.4124 0.0604 -0.9260 0.0140
457 -0.4124 0.0604 -0.9260 0.0140
458 -0.4124 0.0604 -0.9260 0.0140
459 -0.4124 0.0604 -0.9260 0.0140
460 -0.4124 0.0604 -0.9260 0.0140
461 -0.4124 0.0604 -0.9260 0.0140
462 -0.4124 0.0604 -0.9260 0.0140
463 -0.4124 0.0604 -0.9260 0.0140
464 -0.4124 0.0604 -0.9260 0.0140
465 -0.4124 0.0604 -0.9260 0.0140
466 -0.4124 0.0604 -0.9260 0.0140
467 -0.4124 0.0604 -0.9261 0.0140
468 -0.4124 0.0604 -0.9261 0.0140
469 -0.4124 0.0604 -0.9261 0.0140
470 -0.4124 0.0604 -0.9261 0.0140
471 -0.4124 0.0604 -0.9261 0.0140
472 -0.4124 0.0604 -0.9261 0.0140
473 -0.4124 0.0604 -0.9261 0.0140
474 -0.4124 0.0604 -0.9261 0.0140
475 -0.4124 0.0604 -0.9261 0.0140
476 -0.4124 0.0604 -0.9261 0.0140
477 -0.4124 0.0604 -0.9261 0.0140
478 -0.4124 0.0604 -0.9261 0.0139
479 -0.4124 0.0604 -0.9261 0.0139
480 -0.4124 0.0604 -0.9261 0.0139
481 -0.4124 0.0604 -0.9261 0.0139
482 -0.4124 0.0604 -0.9261 0.0139
483 -0.4124 0.0604 -0.9261 0.0139
484 -0.4124 0.0604 -0.9261 0.0139
485 -0.4124 0.0604 -0.9261 0.0139
486 -0.4124 0.0604 -0.9261 0.0139
487 -0.4124 0.0604 -0.9261 0.0139
488 -0.4124 0.0604 -0.9262 0.0139
489 -0.4124 0.0604 -0.9262 0.0139
490 -0.4124 0.0604 -0.9262 0.0139
491 -0.4124 0.0604 -0.9262 0.0139
492 -0.4124 0.0604 -0.9262 0.0139
493 -0.4124 0.0604 -0.9262 0.0139
494 -0.4124 0.0604 -0.9262 0.0139
495 -0.4124 0.0604 -0.9262 0.0139
496 -0.4124 0.0604 -0.9262 0.0139
497 -0.4124 0.0604 -0.9262 0.0139
498 -0.4124 0.0604 -0.9262 0.0139
499 -0.4124 0.0604 -0.9262 0.0139

==> data/scenario1.tex <==
param deepwalk dgi diffpool km mgcn2 mincut ortho sbm deepwalk_low dgi_low diffpool_low km_low mgcn2_low mincut_low ortho_low sbm_low deepwalk_high dgi_high diffpool_high km_high mgcn2_high mincut_high ortho_high sbm_high shchur shchur_low shchur_high agc agc_low agc_high sdcn sdcn_low sdcn_high daegc daegc_low daegc_high
1.0 68.4624 67.4656 61.7162 66.9742 99.8572 100.0000 55.5089 69.5368 68.3353 67.4075 61.4773 66.8840 99.5788 100.0000 55.0561 69.2860 68.5895 67.5237 61.9552 67.0645 100.0000 100.0000 55.9616 69.7877 81.7214 81.6468 81.7960 32.2749 32.2112 32.3386 42.8294 42.6280 43.0308 62.4996 62.3026 62.6966
1.2 68.4525 67.3822 60.8092 67.0451 99.9312 99.8945 55.4547 69.4037 68.3237 67.3409 60.5407 66.9856 99.8893 99.7701 54.9965 69.1946 68.5813 67.4235 61.0777 67.1047 99.9731 100.0000 55.9128 69.6129 81.8381 81.7668 81.9095 30.6769 30.6198 30.7340 42.0683 41.8700 42.2665 54.4047 54.1983 54.6111
1.4 68.2328 67.4673 59.9453 67.0612 100.0000 98.9446 55.7167 69.1504 68.0838 67.4031 59.6670 66.9708 100.0000 97.9050 55.3074 68.9190 68.3818 67.5315 60.2236 67.1515 100.0000 99.9842 56.1261 69.3817 79.7310 79.6602 79.8018 29.3692 29.3041 29.4344 39.8479 39.6534 40.0423 52.8369 52.6350 53.0388
1.6 68.1536 67.3608 58.8464 66.9917 99.9199 95.4887 56.3138 68.9448 67.9973 67.2945 58.5307 66.8862 99.8852 91.5950 55.8254 68.7660 68.3100 67.4270 59.1622 67.0971 99.9546 99.3825 56.8021 69.1235 79.5968 79.5280 79.6657 29.2294 29.1719 29.2870 39.1016 38.9142 39.2890 52.2417 52.0254 52.4580
1.8 67.2430 67.2753 57.8740 67.2155 99.8678 58.6784 56.2958 68.9268 67.0785 67.2242 57.5599 67.1501 99.8154 49.0904 55.7739 68.7148 67.4075 67.3263 58.1882 67.2809 99.9202 68.2665 56.8178 69.1389 76.5171 76.4436 76.5906 27.3984 27.3215 27.4753 36.5302 36.3559 36.7045 44.1817 44.0002 44.3631
2.0 66.5530 67.1248 56.3234 66.9223 99.7666 5.5611 56.0982 68.4504 66.3572 67.0511 56.0579 66.8315 99.7180 1.1848 55.6315 68.2622 66.7487 67.1985 56.5888 67.0131 99.8153 9.9375 56.5649 68.6387 74.8179 74.7539 74.8819 27.8503 27.7811 27.9195 37.4210 37.2575 37.5845 45.7889 45.6241 45.9536
2.2 65.0953 66.8111 54.4325 66.9308 99.2922 0.0000 56.1571 67.9760 64.8653 66.7445 54.1578 66.8048 99.2183 0.0000 55.7053 67.7460 65.3253 66.8777 54.7071 67.0568 99.3662 0.0000 56.6089 68.2059 72.5600 72.4976 72.6223 27.7703 27.6902 27.8503 37.3091 37.1447 37.4735 44.6435 44.4621 44.8248
2.4 63.2740 66.6657 53.2987 67.1430 99.2832 0.0075 56.8856 67.4049 63.0161 66.5968 53.0190 67.0725 99.1879 0.0000 56.4595 67.2042 63.5320 66.7345 53.5785 67.2135 99.3786 0.0189 57.3117 67.6055 70.6107 70.5490 70.6724 25.7093 25.6222 25.7965 33.9102 33.7297 34.0908 41.6598 41.4862 41.8335
2.6 59.9542 66.3268 51.1327 67.0779 98.5566 0.0012 55.8100 66.3073 59.5752 66.2442 50.8004 67.0018 98.4051 0.0000 55.3542 66.0414 60.3331 66.4093 51.4649 67.1541 98.7081 0.0036 56.2658 66.5732 67.3621 67.2911 67.4331 22.4885 22.4072 22.5699 30.6086 30.4386 30.7787 41.0896 40.9582 41.2209
2.8 56.7541 65.9631 49.3902 66.9377 98.3135 0.0060 56.6496 65.2739 56.3597 65.8719 49.0695 66.8563 98.1148 0.0000 56.1043 65.0248 57.1485 66.0544 49.7109 67.0190 98.5121 0.0147 57.1948 65.5231 63.7718 63.7156 63.8281 23.7816 23.7109 23.8523 31.3527 31.1960 31.5094 38.4830 38.3711 38.5948
3.0 51.6854 65.1249 46.9587 67.0943 96.6107 -0.0000 56.5518 62.9850 51.2556 64.9960 46.6368 67.0151 96.4355 0.0000 56.1250 62.6983 52.1151 65.2538 47.2807 67.1734 96.7859 -0.0000 56.9785 63.2716 61.6324 61.5631 61.7018 23.6313 23.5776 23.6849 28.1746 28.0425 28.3067 40.5063 40.4030 40.6095
3.2 45.3080 64.5077 44.6523 66.8536 95.4534 -0.0000 55.9803 60.1744 44.6415 64.3266 44.2933 66.6811 95.0689 0.0000 55.4553 59.8582 45.9746 64.6889 45.0112 67.0261 95.8380 -0.0000 56.5054 60.4906 57.4077 57.3368 57.4786 22.8984 22.8336 22.9633 29.0521 28.9093 29.1949 40.9440 40.8613 41.0266
3.4 37.4849 63.2919 41.3075 66.9845 92.5622 -0.0000 55.5374 55.5484 36.8113 63.1493 40.9491 66.9144 92.1295 0.0000 55.1155 55.0693 38.1585 63.4345 41.6660 67.0546 92.9949 -0.0000 55.9593 56.0274 52.2829 52.2169 52.3488 20.9307 20.8698 20.9916 24.0284 23.9085 24.1483 35.9120 35.8009 36.0230
3.6 31.3738 62.8330 39.8783 67.0717 89.9534 0.0031 56.0550 49.0596 30.7177 62.6511 39.5380 66.9933 89.4881 0.0000 55.6537 48.5644 32.0299 63.0149 40.2187 67.1502 90.4187 0.0092 56.4563 49.5549 48.3232 48.2656 48.3808 21.9333 21.8537 22.0128 24.1000 23.9664 24.2336 35.7919 35.6686 35.9151
3.8 21.9778 61.2902 36.7510 67.1513 85.6873 0.0026 55.5027 32.7965 21.2308 61.0397 36.3719 67.0946 85.3061 0.0000 55.0634 31.4419 22.7249 61.5406 37.1300 67.2080 86.0685 0.0077 55.9420 34.1512 44.3375 44.2788 44.3961 21.7552 21.7103 21.8001 22.4882 22.3886 22.5879 28.9156 28.8408 28.9903
4.0 15.6291 58.7014 34.0823 67.0503 79.9469 -0.0000 55.0146 18.1582 14.9993 58.3787 33.7065 66.9830 79.3931 0.0000 54.4911 17.0366 16.2589 59.0241 34.4582 67.1175 80.5007 -0.0000 55.5380 19.2799 37.8068 37.7295 37.8840 19.3196 19.2643 19.3749 19.0082 18.9110 19.1054 28.0123 27.8991 28.1255
4.2 10.7583 57.1539 32.0474 67.1251 74.5584 -0.0000 55.0580 9.7619 10.2749 56.9276 31.6109 67.0667 74.1867 0.0000 54.6027 8.9794 11.2416 57.3803 32.4838 67.1835 74.9300 -0.0000 55.5133 10.5445 34.3011 34.2470 34.3553 20.1185 20.0550 20.1821 17.8749 17.7807 17.9691 24.3522 24.2451 24.4592
4.4 8.1352 54.2879 28.7726 67.0047 70.2869 0.0022 53.6921 4.8346 7.7911 53.9564 28.4033 66.9316 69.6524 0.0000 53.2072 4.5241 8.4792 54.6194 29.1419 67.0777 70.9214 0.0064 54.1771 5.1451 29.2608 29.2185 29.3032 18.8732 18.8157 18.9307 16.0933 16.0144 16.1721 22.4048 22.3460 22.4636
4.6 5.5535 51.0879 25.9074 67.0652 64.3963 0.0000 54.8372 2.9431 5.3123 50.6080 25.5919 66.9890 63.8361 0.0000 54.3126 2.7869 5.7946 51.5677 26.2228 67.1414 64.9565 0.0000 55.3619 3.0993 23.8088 23.7610 23.8566 17.4897 17.4418 17.5377 14.2129 14.1339 14.2920 16.6429 16.6002 16.6857
4.8 4.3036 48.0695 24.0403 67.0921 57.3425 0.0000 53.8947 2.3908 4.1384 47.7001 23.6559 67.0145 56.8766 0.0000 53.3262 2.2433 4.4688 48.4388 24.4247 67.1697 57.8083 0.0000 54.4632 2.5384 20.2042 20.1666 20.2418 18.1967 18.1422 18.2513 13.2597 13.1903 13.3291 16.8402 16.7825 16.8980
5.0 3.4444 44.0793 20.7364 67.1758 51.1604 0.0019 54.4826 1.8811 3.3040 43.6741 20.3701 67.1108 50.6383 0.0000 54.0095 1.7868 3.5849 44.4844 21.1027 67.2408 51.6825 0.0057 54.9558 1.9755 15.9906 15.9628 16.0184 16.9968 16.9646 17.0290  13.6836 13.6190 13.7482

==> data/scenario2.tex <==
param deepwalk dgi diffpool km mgcn2 mincut ortho sbm deepwalk_low dgi_low diffpool_low km_low mgcn2_low mincut_low ortho_low sbm_low deepwalk_high dgi_high diffpool_high km_high mgcn2_high mincut_high ortho_high sbm_high shchur shchur_low shchur_high agc agc_low agc_high sdcn sdcn_low sdcn_high daegc daegc_low daegc_high
0.01 66.6553 35.2439 46.7701 2.7919 76.4178 0.0047 14.2236 68.5019 66.4672 34.6300 46.3675 2.6660 75.8280 0.0000 13.7146 68.3309 66.8433 35.8578 47.1727 2.9178 77.0076 0.0139 14.7325 68.6730 68.9328 68.8243 69.0414 5.7186 5.6901 5.7471 8.8999 8.8338 8.9661 25.8074 25.7266 25.8882
0.02 66.6684 42.4897 48.6696 3.3548 83.0598 0.0120 18.6443 68.5382 66.4861 41.7545 48.2827 3.2242 82.3896 0.0000 18.0091 68.3234 66.8507 43.2249 49.0565 3.4854 83.7300 0.0248 19.2795 68.7530 73.8132 73.7313 73.8951 7.2721 7.2394 7.3047 12.4295 12.3446 12.5144 29.8895 29.7793 29.9997
0.03 66.6793 49.9945 50.5723 5.1700 89.7162 0.0119 24.7878 68.5525 66.4841 49.3438 50.2261 4.9135 88.9967 0.0000 24.2033 68.3466 66.8746 50.6451 50.9185 5.4266 90.4356 0.0273 25.3724 68.7583 75.2358 75.1645 75.3071 9.4133 9.3658 9.4608 15.6488 15.5538 15.7437 32.6911 32.5693 32.8128
0.04 66.5608 55.1122 52.1638 7.9019 93.1260 0.0006 29.9850 68.6841 66.3565 54.7085 51.8596 7.6828 92.7615 0.0000 29.5151 68.4761 66.7651 55.5159 52.4679 8.1209 93.4905 0.0017 30.4549 68.8921 75.1816 75.1094 75.2537 14.7903 14.7471 14.8336 24.7296 24.6149 24.8443 37.1755 37.0785 37.2725
0.06 66.5076 60.0764 53.9516 12.2849 96.2179 0.0024 35.8063 68.2507 66.3344 59.6304 53.5773 11.7535 95.8590 0.0000 35.1203 68.0626 66.6808 60.5224 54.3259 12.8162 96.5769 0.0072 36.4923 68.4388 75.9898 75.9024 76.0773 18.0402 17.9593 18.1211 29.1192 28.9459 29.2926 44.9182 44.7820 45.0544
0.09 66.8176 62.8188 55.0583 17.9038 98.8165 0.0003 39.9947 68.7468 66.6083 62.6160 54.7701 17.5073 98.6638 0.0000 39.5547 68.5353 67.0269 63.0216 55.3466 18.3002 98.9691 0.0009 40.4346 68.9582 75.4712 75.4027 75.5397 25.7247 25.6444 25.8051 35.4449 35.2440 35.6457 46.0629 45.9262 46.1995
0.13 66.7558 65.1407 55.5161 29.3573 99.2467 0.0089 45.1147 68.4549 66.5544 64.9966 55.2424 28.8075 99.1145 0.0000 44.6426 68.2787 66.9573 65.2848 55.7897 29.9070 99.3790 0.0190 45.5868 68.6311 74.3857 74.3205 74.4508 32.2725 32.2126 32.3323 39.8615 39.6885 40.0344 46.2641 46.1127 46.4155
0.18 66.3355 66.1383 55.6720 40.7953 99.4186 0.0126 47.5961 68.7355 66.1359 66.0041 55.3900 40.2061 99.3359 0.0004 47.1859 68.5277 66.5350 66.2726 55.9541 41.3845 99.5012 0.0248 48.0063 68.9433 74.8586 74.7994 74.9178 40.1100 40.0131 40.2070 48.7810 48.5971 48.9650 52.1713 51.9934 52.3491
0.26 66.4069 66.4439 56.1177 50.1923 99.6724 0.0015 49.9932 68.7180 66.2184 66.3638 55.8338 49.5815 99.5878 0.0000 49.5494 68.5036 66.5954 66.5240 56.4017 50.8030 99.7570 0.0044 50.4370 68.9325 76.2875 76.2195 76.3556 49.3523 49.2777 49.4269 52.6333 52.4441 52.8225 59.2071 58.9927 59.4214
0.38 66.8428 66.9164 56.3537 60.7260 99.7126 0.0060 51.8531 68.4335 66.6586 66.8554 56.0943 60.0438 99.6471 0.0000 51.3549 68.2251 67.0271 66.9774 56.6132 61.4081 99.7781 0.0178 52.3513 68.6419 75.6327 75.5719 75.6935 55.4213 55.3569 55.4856 59.2730 59.0809 59.4652 60.0709 59.8820 60.2597
0.55 66.6547 67.0265 56.5579 64.0882 99.8608 1.9369 53.2517 68.5405 66.4505 66.9632 56.2774 63.5732 99.8179 0.0000 52.7745 68.3457 66.8589 67.0899 56.8385 64.6032 99.9037 4.5884 53.7289 68.7353 76.2859 76.2373 76.3345 59.8801 59.8388 59.9214 61.6513 61.4518 61.8507 65.2027 65.0390 65.3664
0.78 66.3076 66.9666 56.9866 66.5129 99.7814 -0.0000 54.9630 68.4617 66.1190 66.8871 56.7289 66.3908 99.7068 0.0000 54.4798 68.2509 66.4963 67.0460 57.2443 66.6350 99.8559 -0.0000 55.4461 68.6724 77.0543 76.9935 77.1150 61.8805 61.8491 61.9119 64.5118 64.3251 64.6985 67.0628 66.8663 67.2594
1.13 66.6793 67.1133 56.7245 67.1845 99.6413 15.8871 56.8112 68.6068 66.4729 67.0518 56.4066 67.1253 99.5711 8.7521 56.3375 68.3968 66.8857 67.1749 57.0424 67.2438 99.7114 23.0220 57.2849 68.8167 77.0459 76.9948 77.0970 63.9230 63.8951 63.9509 69.4019 69.2189 69.5848 69.4035 69.2115 69.5955
1.62 66.4560 67.2240 56.2723 67.2967 99.7607 49.8310 58.5168 68.8019 66.2945 67.1433 55.9932 67.2375 99.6990 40.0640 58.1040 68.6138 66.6175 67.3047 56.5515 67.3558 99.8225 59.5980 58.9295 68.9899 77.0861 77.0396 77.1326 64.6705 64.6466 64.6943 73.6446 73.4468 73.8425 73.4588 73.2551 73.6624
2.34 66.7112 67.2887 56.0359 67.2525 99.9484 69.8353 60.3376 68.6787 66.5039 67.2367 55.6837 67.2074 99.9196 60.8744 59.8144 68.4810 66.9185 67.3406 56.3882 67.2976 99.9771 78.7961 60.8608 68.8763 77.5092 77.4502 77.5682 64.8282 64.8057 64.8507 78.1741 77.9507 78.3975 70.7300 70.5137 70.9463
3.36 66.7414 67.3835 56.3723 67.2942 99.8053 88.6378 61.2939 68.5844 66.5214 67.3129 55.8929 67.2391 99.7472 82.5297 60.8130 68.3681 66.9615 67.4540 56.8518 67.3493 99.8634 94.7460 61.7748 68.8006 77.5826 77.5224 77.6429 65.7106 65.6953 65.7259 85.9392 85.7653 86.1131 73.8704 73.7133 74.0275
4.83 66.4890 67.3825 58.2407 67.2720 99.3334 95.6383 62.0283 68.4879 66.2925 67.3334 57.5687 67.2207 98.7610 91.8111 61.5097 68.2940 66.6854 67.4317 58.9127 67.3233 99.9059 99.4655 62.5470 68.6818 77.3042 77.2520 77.3565 65.9169 65.9037 65.9301 89.1133 88.9897 89.2368 70.1216 69.9105 70.3327
6.95 66.5014 67.2246 58.9922 67.3082 99.1783 95.4421 62.3189 68.4712 66.3333 67.1441 58.2563 67.2537 98.6244 91.6229 61.8497 68.2740 66.6696 67.3050 59.7281 67.3628 99.7322 99.2612 62.7882 68.6684 77.9988 77.9341 78.0634 65.9421 65.9276 65.9565 87.7957 87.6634 87.9280 73.6925 73.5257 73.8594
10.0 66.6193 67.3720 61.1372 67.3037 99.0826 96.7216 63.0360 68.9319 66.4517 67.3195 60.5267 67.2501 98.4790 93.3871 62.4509 68.6976 66.7869 67.4246 61.7477 67.3573 99.6861 100.0000 63.6211 69.1662 76.9608 76.9018 77.0197 65.9830 65.9689 65.9972 88.9026 88.8112 88.9941 68.5746 68.3763 68.7730

==> data/scenario3.tex <==
param deepwalk dgi diffpool km mgcn2 mincut ortho sbm deepwalk_low dgi_low diffpool_low km_low mgcn2_low mincut_low ortho_low sbm_low deepwalk_high dgi_high diffpool_high km_high mgcn2_high mincut_high ortho_high sbm_high shchur shchur_low shchur_high agc agc_low agc_high sdcn sdcn_low sdcn_high daegc daegc_low daegc_high
0.01 66.4328 28.8984 44.3898 2.3420 67.8034 0.0007 11.1234 68.5936 66.2533 28.0229 43.8948 2.2513 66.7931 0.0000 10.6007 68.3980 66.6124 29.7739 44.8847 2.4326 68.8137 0.0019 11.6461 68.7893 64.9392 64.8407 65.0376 4.7300 4.7083 4.7516 6.8906 6.8350 6.9461 22.7239 22.6158 22.8319
0.02 66.5421 34.7312 45.9085 2.9463 73.4672 0.0024 14.1401 68.6711 66.3478 33.8142 45.3729 2.7944 72.5236 0.0000 13.5030 68.4791 66.7365 35.6483 46.4440 3.0981 74.4108 0.0071 14.7773 68.8632 69.5775 69.4716 69.6834 5.7840 5.7641 5.8039 9.8379 9.7616 9.9142 29.0964 28.9852 29.2076
0.03 66.2202 41.8693 47.9421 3.8286 81.2907 0.0090 18.7421 68.4599 66.0088 41.1260 47.5874 3.6796 80.4978 0.0000 18.1410 68.2185 66.4316 42.6126 48.2969 3.9777 82.0837 0.0212 19.3432 68.7013 73.7811 73.6903 73.8720 8.2477 8.2075 8.2880 12.2383 12.1357 12.3408 32.0133 31.9116 32.1149
0.04 66.5494 49.9012 50.5477 5.1776 89.0171 0.0052 25.0347 68.9938 66.3819 49.4742 50.2510 4.9817 88.5372 0.0000 24.5602 68.7951 66.7169 50.3281 50.8443 5.3736 89.4970 0.0153 25.5092 69.1925 76.0593 75.9807 76.1379 10.1329 10.0944 10.1713 16.9885 16.8759 17.1010 31.7594 31.6633 31.8555
0.06 66.7600 56.1807 52.4424 9.0281 94.0345 0.0017 31.2479 68.6548 66.5781 55.6718 52.1102 8.7247 93.5032 0.0000 30.7053 68.4537 66.9419 56.6897 52.7747 9.3316 94.5658 0.0050 31.7906 68.8558 75.1134 75.0387 75.1882 14.2021 14.1603 14.2439 21.9253 21.7871 22.0635 40.0068 39.8841 40.1295
0.09 66.2717 59.0917 53.3830 14.3278 95.1195 0.0190 35.3668 68.4724 66.0793 58.6448 53.0880 13.7932 94.5482 0.0000 34.7688 68.2424 66.4641 59.5386 53.6779 14.8623 95.6908 0.0522 35.9648 68.7025 75.4708 75.3980 75.5437 19.5662 19.4928 19.6396 28.7814 28.6255 28.9374 41.0008 40.8954 41.1062
0.13 66.3943 62.8888 54.6926 24.7910 98.1361 0.0296 40.7290 68.4553 66.2277 62.5468 54.3461 23.8853 97.7616 0.0022 40.0217 68.2654 66.5609 63.2308 55.0391 25.6967 98.5106 0.0569 41.4363 68.6451 75.0801 75.0097 75.1504 29.0979 29.0345 29.1613 36.0585 35.8931 36.2239 46.4370 46.2662 46.6079
0.18 66.5091 64.3892 55.0345 32.6221 97.9409 0.0020 43.5117 68.6579 66.3186 64.1871 54.7092 31.7421 97.3371 0.0000 42.9724 68.4521 66.6997 64.5912 55.3598 33.5020 98.5448 0.0058 44.0509 68.8638 73.6931 73.6302 73.7560 39.8152 39.7317 39.8988 41.0366 40.8797 41.1934 50.8259 50.6524 50.9995
0.26 66.5105 65.9846 56.4111 48.0076 99.5752 0.0155 48.2842 68.4953 66.3059 65.8879 56.1374 47.0443 99.5197 0.0000 47.8360 68.2804 66.7152 66.0814 56.6848 48.9709 99.6307 0.0328 48.7325 68.7102 75.4526 75.3897 75.5155 48.8861 48.8201 48.9521 45.2097 45.0226 45.3969 54.1337 53.9529 54.3144
0.38 66.4076 66.4005 56.3025 57.7115 99.6636 0.0077 50.3135 68.7370 66.2127 66.2904 56.0148 57.0210 99.5907 0.0000 49.8764 68.4951 66.6024 66.5107 56.5902 58.4021 99.7366 0.0184 50.7506 68.9788 74.4632 74.4086 74.5178 55.6818 55.6069 55.7567 50.6253 50.4337 50.8169 59.5073 59.2575 59.7571
0.55 66.2175 66.7025 56.2784 64.5711 99.5292 0.0027 52.9066 68.2405 66.0156 66.6258 56.0300 64.1459 99.4458 0.0000 52.4414 68.0337 66.4194 66.7793 56.5268 64.9964 99.6127 0.0068 53.3717 68.4473 75.7601 75.7083 75.8120 61.6561 61.6101 61.7021 53.1560 52.9727 53.3394 62.7871 62.5657 63.0086
0.78 66.6489 67.0095 56.9638 66.7003 99.8539 0.0019 54.9640 68.6910 66.4537 66.9404 56.7057 66.5847 99.8112 0.0000 54.5177 68.4993 66.8440 67.0786 57.2218 66.8160 99.8967 0.0046 55.4103 68.8828 74.7448 74.6865 74.8031 63.7958 63.7679 63.8236 55.7856 55.6076 55.9637 63.8021 63.6040 64.0003
1.13 66.3778 66.8633 56.6607 67.3841 99.3968 2.5636 55.4023 68.2934 66.2309 66.7973 56.3668 67.2993 99.3048 0.0000 54.9316 68.0998 66.5248 66.9292 56.9546 67.4688 99.4888 5.4853 55.8731 68.4870 75.4034 75.3471 75.4596 65.5726 65.5564 65.5888 60.1139 59.9576 60.2702 62.6168 62.3759 62.8577
1.62 66.4811 67.1973 56.4392 67.5457 99.7348 29.1181 57.3107 68.3892 66.2919 67.1247 56.0907 67.4794 99.6647 20.4773 56.8067 68.1620 66.6703 67.2699 56.7876 67.6120 99.8049 37.7588 57.8146 68.6164 74.8888 74.8286 74.9489 66.4775 66.4666 66.4883 61.5242 61.3408 61.7076 68.7307 68.5468 68.9145
2.34 66.4712 67.3085 56.4998 67.4793 99.7427 41.0237 57.2874 68.4631 66.2796 67.2456 56.1640 67.4081 99.6887 31.6463 56.9037 68.2571 66.6628 67.3714 56.8356 67.5505 99.7966 50.4011 57.6712 68.6691 75.4416 75.3890 75.4942 66.8141 66.8051 66.8230 74.6741 74.4607 74.8876 67.7692 67.5525 67.9859
3.36 66.4729 67.2221 56.2006 67.5402 99.6232 87.6938 57.6631 68.7182 66.2768 67.1583 55.8756 67.4806 99.5460 81.5806 57.1394 68.5136 66.6691 67.2859 56.5255 67.5999 99.7004 93.8069 58.1868 68.9229 75.1688 75.1227 75.2150 66.9622 66.9538 66.9705 78.0888 77.9124 78.2652 69.3759 69.1641 69.5878
4.83 66.6859 67.2921 56.3010 67.5913 99.5810 92.3779 58.4173 68.6846 66.5045 67.2124 55.8819 67.5169 99.5309 87.4075 57.8937 68.4982 66.8674 67.3719 56.7202 67.6658 99.6310 97.3483 58.9409 68.8710 75.5474 75.4905 75.6043 66.9797 66.9719 66.9875 76.6151 76.4295 76.8007 69.0229 68.8514 69.1944
6.95 66.4120 67.4146 57.4358 67.5084 99.6831 92.1055 58.7812 68.5332 66.2188 67.3391 56.9530 67.4473 99.6054 87.0862 58.2629 68.3171 66.6053 67.4902 57.9186 67.5695 99.7608 97.1248 59.2995 68.7493 76.0316 75.9759 76.0873 67.0727 67.0663 67.0792 78.7596 78.5914 78.9277 70.4278 70.2549 70.6007
10.0 66.8328 67.4579 57.7403 67.5577 99.3864 97.5755 58.8227 68.5552 66.6592 67.3882 57.2210 67.4847 98.8908 94.8315 58.3829 68.3694 67.0065 67.5276 58.2597 67.6307 99.8820 100.0000 59.2625 68.7410 76.2363 76.1745 76.2980 66.9440 66.9375 66.9506 80.7109 80.5950 80.8268 65.0461 64.8393 65.2528

==> data/scenario4.tex <==
param deepwalk dgi diffpool km mgcn2 mincut ortho sbm deepwalk_low dgi_low diffpool_low km_low mgcn2_low mincut_low ortho_low sbm_low deepwalk_high dgi_high diffpool_high km_high mgcn2_high mincut_high ortho_high sbm_high shchur shchur_low shchur_high agc agc_low agc_high sdcn sdcn_low sdcn_high daegc daegc_low daegc_high
0.01 66.6113 28.8745 41.6895 2.5457 62.6784 0.0072 12.4721 68.8051 66.4154 28.0342 41.1221 2.4161 61.2845 0.0000 11.8706 68.5834 66.8072 29.7147 42.2569 2.6753 64.0722 0.0154 13.0736 69.0268 61.2019 61.0733 61.3304 4.5482 4.5269 4.5695 8.5195 8.4401 8.5989 26.4371 26.3456 26.5286
0.02 66.5387 35.0493 43.0138 3.1031 70.0164 0.0070 16.2590 68.6442 66.3405 34.3089 42.5613 2.9529 68.9859 0.0000 15.6872 68.4112 66.7369 35.7896 43.4662 3.2533 71.0470 0.0150 16.8309 68.8771 65.4910 65.3920 65.5900 5.9310 5.9083 5.9536 10.4579 10.3782 10.5376 24.1337 24.0636 24.2038
0.03 66.5963 39.5989 44.1363 4.6611 74.0511 0.0099 20.1421 68.5116 66.4089 38.9955 43.7661 4.4112 73.3991 0.0001 19.5608 68.3463 66.7836 40.2023 44.5064 4.9110 74.7031 0.0197 20.7234 68.6769 66.5975 66.5042 66.6908 8.0165 7.9925 8.0405 15.3280 15.2309 15.4252 27.8101 27.6934 27.9268
0.04 66.4136 43.5932 44.9725 6.8810 77.8363 0.0022 23.9641 68.5192 66.1963 43.1528 44.5754 6.4969 77.3803 0.0000 23.3923 68.3104 66.6308 44.0336 45.3697 7.2651 78.2924 0.0065 24.5358 68.7280 66.0535 65.9713 66.1358 10.7509 10.7090 10.7928 20.4421 20.2908 20.5933 34.4678 34.3507 34.5849
0.06 66.4131 45.6216 45.7461 9.4740 80.5762 0.0083 26.6385 68.4980 66.2254 45.2157 45.3248 9.0471 80.1843 0.0000 26.1784 68.2892 66.6007 46.0275 46.1674 9.9009 80.9682 0.0210 27.0986 68.7067 67.1658 67.0918 67.2397 12.7243 12.6908 12.7579 23.1775 23.0278 23.3272 32.7205 32.6477 32.7933
0.09 66.6761 48.8216 46.0800 16.3905 82.5005 0.0057 31.4035 68.5597 66.4845 48.4944 45.7190 15.7125 82.1429 0.0000 30.8932 68.3529 66.8676 49.1488 46.4410 17.0685 82.8582 0.0139 31.9137 68.7665 67.0596 66.9867 67.1326 17.0745 17.0327 17.1162 29.9352 29.7649 30.1055 34.8623 34.7418 34.9829
0.13 66.4753 49.9312 45.3705 24.9044 82.8267 -0.0000 34.5780 68.6341 66.2983 49.7281 44.9399 24.1905 82.4304 0.0000 34.2126 68.4450 66.6522 50.1342 45.8010 25.6182 83.2231 -0.0000 34.9434 68.8233 66.1791 66.1042 66.2540 21.6633 21.6055 21.7211 33.4313 33.2686 33.5941 34.0823 33.9496 34.2150
0.18 66.6947 50.1709 44.7725 30.0184 83.4688 0.0012 35.2150 68.6311 66.5203 50.0172 44.4480 29.2730 83.2117 0.0000 34.8303 68.4111 66.8691 50.3245 45.0971 30.7638 83.7258 0.0033 35.5997 68.8511 67.3097 67.2138 67.4055 26.2265 26.1508 26.3022 39.2813 39.1031 39.4594 35.1157 34.9890 35.2424
0.26 66.5876 50.7383 44.2681 39.4167 84.4023 0.0040 37.2198 68.6395 66.3939 50.5893 43.9416 38.6935 84.1903 0.0000 36.8521 68.4233 66.7812 50.8872 44.5946 40.1398 84.6143 0.0096 37.5874 68.8557 65.8989 65.8188 65.9790 30.3456 30.2828 30.4084 42.6597 42.4708 42.8486 34.5522 34.4149 34.6896
0.38 66.4497 50.8387 44.4262 46.0833 84.6647 0.0099 39.2371 68.6583 66.2553 50.6965 44.1140 45.7150 84.3606 0.0000 38.8293 68.4557 66.6441 50.9809 44.7384 46.4517 84.9687 0.0236 39.6449 68.8610 65.8914 65.8010 65.9818 35.8217 35.7666 35.8769 47.7368 47.5515 47.9221 34.9205 34.7646 35.0764
0.55 66.6673 51.0159 45.0365 48.8297 84.3865 0.0000 40.1162 68.5464 66.4892 50.8946 44.7434 48.5898 84.1519 0.0000 39.7250 68.3433 66.8455 51.1372 45.3295 49.0696 84.6211 0.0000 40.5074 68.7495 65.1040 65.0235 65.1845 38.2057 38.1514 38.2600 50.1003 49.9297 50.2709 40.0207 39.7852 40.2561
0.78 66.6956 50.9554 45.1005 50.1499 83.3854 0.0068 41.2151 68.6467 66.4955 50.8079 44.7579 50.0312 82.9128 0.0000 40.8397 68.4234 66.8956 51.1029 45.4430 50.2687 83.8580 0.0200 41.5904 68.8700 64.0169 63.9406 64.0931 40.5636 40.5163 40.6109 53.8825 53.7251 54.0400 40.5635 40.3334 40.7936
1.13 66.2224 50.2975 43.8811 50.0692 82.1077 -0.0000 42.3431 68.3470 66.0235 50.1729 43.5222 49.9708 81.6981 0.0000 42.0088 68.1591 66.4212 50.4221 44.2399 50.1675 82.5174 -0.0000 42.6775 68.5348 66.1590 66.0522 66.2658 41.9947 41.9498 42.0395 53.8458 53.6883 54.0034 34.9727 34.7709 35.1745
1.62 66.5080 50.6990 43.0556 50.4846 82.9008 4.1885 44.5826 68.7020 66.3053 50.6144 42.6427 50.4063 82.6137 0.6101 44.1446 68.5053 66.7107 50.7836 43.4686 50.5629 83.1880 7.7669 45.0206 68.8988 67.5432 67.4577 67.6288 43.3730 43.3325 43.4135 59.4222 59.2422 59.6021 47.7044 47.5160 47.8929
2.34 66.7208 50.7815 43.2703 50.5674 83.7235 3.4255 45.5470 68.6736 66.5638 50.6561 42.7600 50.4740 83.2356 0.1362 45.0542 68.4499 66.8777 50.9070 43.7807 50.6609 84.2113 6.7149 46.0398 68.8973 64.4510 64.3796 64.5223 44.0292 43.9948 44.0636 66.2674 66.0614 66.4735 53.2110 52.9028 53.5192
3.36 66.5987 50.6911 44.3372 50.4722 82.6103 16.1404 46.4220 68.5682 66.4322 50.5651 43.7421 50.3632 82.3233 9.6083 45.9571 68.3681 66.7652 50.8170 44.9323 50.5812 82.8972 22.6725 46.8868 68.7683 61.8295 61.7617 61.8973 44.8349 44.8023 44.8676 69.4965 69.3275 69.6654 60.8941 60.7045 61.0837
4.83 66.7434 51.2639 45.8876 50.8102 83.7907 35.8900 47.7066 68.7006 66.5712 51.1646 45.2707 50.7232 83.3347 27.6229 47.2880 68.4764 66.9157 51.3631 46.5045 50.8971 84.2467 44.1572 48.1252 68.9248 61.0800 61.0068 61.1531 44.8556 44.8264 44.8848 72.0243 71.8952 72.1534 59.0539 58.8174 59.2904
6.95 66.6657 50.6171 46.6186 50.3188 80.7474 24.8028 47.5032 68.6773 66.5032 50.5247 45.9970 50.2329 80.3529 17.1960 47.0336 68.4603 66.8281 50.7095 47.2402 50.4047 81.1420 32.4097 47.9728 68.8942 60.0823 60.0075 60.1570 44.5967 44.5638 44.6295 73.1306 73.0106 73.2506 55.2027 54.9001 55.5054
10.0 66.6379 50.7468 47.5869 50.5082 81.7220 30.7010 48.5954 68.7800 66.4366 50.5818 47.0680 50.3589 80.9848 22.6772 48.0140 68.5999 66.8393 50.9119 48.1059 50.6575 82.4591 38.7248 49.1769 68.9600 59.3142 59.2459 59.3826 45.6134 45.5823 45.6446 71.9478 71.8218 72.0739 57.2775 57.0861 57.4690

==> data/scenario5.tex <==
param deepwalk dgi diffpool km mgcn2 mincut ortho sbm deepwalk_low dgi_low diffpool_low km_low mgcn2_low mincut_low ortho_low sbm_low deepwalk_high dgi_high diffpool_high km_high mgcn2_high mincut_high ortho_high sbm_high shchur shchur_low shchur_high agc agc_low agc_high sdcn sdcn_low sdcn_high daegc daegc_low daegc_high
2.0 7.2057 57.9180 19.8353 67.1809 69.2246 40.0776 45.6385 4.4852 6.9720 57.6677 19.3969 67.1210 68.8324 39.7011 45.2374 4.2657 7.4395 58.1684 20.2737 67.2409 69.6168 40.4541 46.0396 4.7047 19.9998 19.9507 20.0488 18.6997 18.6513 18.7480 13.6246 13.5556 13.6937 9.4440 9.4128 9.4752
2.49 8.0295 57.5770 21.7683 66.9139 69.6096 39.7968 44.7712 5.4149 7.7442 57.3861 21.3862 66.8257 69.0409 39.3781 44.3383 5.1212 8.3147 57.7678 22.1503 67.0021 70.1783 40.2155 45.2041 5.7086 21.2485 21.2144 21.2825 18.5151 18.4801 18.5500 13.6754 13.6133 13.7375 12.0667 12.0361 12.0973
3.1 12.3209 59.0120 25.4025 67.0165 73.5741 41.5553 46.1019 7.5457 11.8321 58.8335 25.0925 66.9404 73.1461 41.2661 45.7742 7.2609 12.8098 59.1904 25.7124 67.0926 74.0021 41.8445 46.4297 7.8304 25.9184 25.8667 25.9702 21.0025 20.9389 21.0662 15.2190 15.1371 15.3009 13.2032 13.1466 13.2598
3.86 19.4610 60.4271 28.5867 66.9999 79.1507 43.6735 47.9667 12.3047 18.6281 60.1770 28.1585 66.9230 78.6312 43.2679 47.6174 11.7687 20.2940 60.6772 29.0148 67.0769 79.6701 44.0791 48.3160 12.8406 29.0338 28.9931 29.0744 23.5562 23.5001 23.6123 18.5569 18.4772 18.6366 14.6604 14.6073 14.7134
4.8 26.5198 61.5223 31.1496 67.0938 82.5657 45.9782 49.6455 18.7955 25.8215 61.3659 30.7642 67.0190 82.1602 45.6303 49.2584 18.1371 27.2181 61.6788 31.5349 67.1687 82.9712 46.3260 50.0327 19.4539 33.4850 33.4371 33.5329 22.8690 22.8019 22.9361 19.4349 19.3439 19.5260 16.8798 16.8013 16.9583
5.98 36.0533 63.0335 35.6421 67.1449 88.0638 48.2045 51.1430 33.3980 35.3235 62.8262 35.2515 67.0736 87.6885 47.9148 50.7499 32.6141 36.7831 63.2408 36.0326 67.2161 88.4391 48.4942 51.5360 34.1819 38.0828 38.0248 38.1409 23.2504 23.1618 23.3391 20.9870 20.8749 21.0990 17.5653 17.5177 17.6129
7.44 43.7418 64.1043 39.3866 67.2005 92.3234 51.0207 53.0886 48.2300 43.1786 63.9726 39.0556 67.1486 91.9866 50.6956 52.6657 47.6759 44.3050 64.2361 39.7177 67.2525 92.6602 51.3458 53.5116 48.7842 45.2115 45.1551 45.2679 25.2514 25.1886 25.3141 23.7110 23.5879 23.8341 24.3407 24.2825 24.3988
9.26 52.3883 65.1017 43.7594 67.0594 94.5954 52.5397 54.0625 58.4636 51.9795 64.9928 43.4141 66.9860 94.1420 51.0272 53.6341 58.1331 52.7971 65.2105 44.1047 67.1328 95.0488 54.0522 54.4909 58.7942 52.5234 52.4743 52.5726 25.6923 25.6416 25.7430 27.3952 27.2671 27.5234 28.0630 27.9641 28.1618
11.52 58.3403 66.2389 47.6162 67.0203 98.0688 38.7370 55.0937 63.2168 58.0370 66.1265 47.2586 66.9229 97.8622 33.6719 54.6165 62.9185 58.6436 66.3514 47.9739 67.1177 98.2754 43.8020 55.5708 63.5150 59.4013 59.3455 59.4571 25.5426 25.4726 25.6127 28.7240 28.5851 28.8630 35.4686 35.3649 35.5723
14.34 62.7606 66.7537 51.5657 67.0617 98.9747 30.5282 55.8805 66.2720 62.5080 66.6700 51.2647 66.9668 98.8598 24.0407 55.4428 66.0426 63.0133 66.8374 51.8666 67.1566 99.0897 37.0156 56.3182 66.5015 66.6194 66.5690 66.6698 27.8068 27.7476 27.8661 33.2476 33.1105 33.3846 37.8971 37.7966 37.9977
17.85 65.6466 67.0530 55.1718 67.0671 99.4751 18.1720 56.3882 68.0038 65.4561 66.9760 54.9032 67.0099 99.3604 11.2342 55.8707 67.8334 65.8372 67.1301 55.4403 67.1243 99.5899 25.1099 56.9056 68.1742 73.3711 73.3102 73.4320 27.5965 27.5237 27.6693 35.6660 35.4814 35.8507 43.3928 43.2615 43.5241
22.22 67.0049 67.0826 57.8400 67.0661 99.7728 5.9836 56.2839 68.6857 66.8144 67.0204 57.6020 66.9799 99.7091 1.3474 55.7840 68.4940 67.1954 67.1448 58.0780 67.1523 99.8364 10.6197 56.7838 68.8774 77.2733 77.2102 77.3365 29.4498 29.3840 29.5156 39.9279 39.7497 40.1060 50.1339 49.9518 50.3161
27.66 68.2588 67.2150 59.9081 67.0987 99.9672 2.0018 56.1288 69.7131 68.1174 67.1616 59.6079 67.0392 99.9437 0.0000 55.6462 69.4828 68.4001 67.2683 60.2084 67.1582 99.9906 4.7458 56.6114 69.9435 80.9879 80.9215 81.0543 27.5737 27.4963 27.6510 40.9352 40.7692 41.1013 53.1590 52.9703 53.3476
34.42 68.6383 67.2564 61.1048 67.1182 100.0000 0.0003 56.1536 69.8810 68.4984 67.2062 60.8674 67.0529 100.0000 0.0000 55.7047 69.6366 68.7781 67.3067 61.3421 67.1835 100.0000 0.0008 56.6025 70.1254 83.1087 83.0364 83.1809 26.8064 26.7179 26.8949 43.8064 43.5836 44.0292 59.3223 59.0392 59.6055
42.84 68.9739 67.2390 62.0617 67.0817 100.0000 2.0000 56.0005 70.0975 68.8383 67.1982 61.8624 66.9839 100.0000 0.0000 55.5062 69.8681 69.1094 67.2797 62.2609 67.1796 100.0000 4.7440 56.4948 70.3269 84.0745 83.9986 84.1505 28.4363 28.3689 28.5037 48.1821 47.9417 48.4225 62.4094 62.1875 62.6312
53.33 69.4358 67.2610 64.1936 67.1816 100.0000 0.0007 56.0746 70.5609 69.2812 67.2115 64.0116 67.0849 100.0000 0.0000 55.5552 70.3114 69.5904 67.3106 64.3755 67.2783 100.0000 0.0021 56.5940 70.8104 83.9398 83.8727 84.0068 29.9918 29.9056 30.0780 52.4288 52.1589 52.6988 67.0942 66.8520 67.3364
66.38 69.8584 67.2396 68.8716 67.0495 100.0000 0.0033 55.7882 70.9128 69.6689 67.1949 68.6496 66.9584 100.0000 0.0000 55.2927 70.6279 70.0479 67.2842 69.0937 67.1406 100.0000 0.0097 56.2837 71.1976 85.7831 85.7112 85.8550 28.0970 27.9988 28.1952 54.9356 54.6982 55.1731 65.8360 65.6284 66.0435
82.62 70.1506 67.2956 77.4184 67.0306 100.0000 -0.0000 56.3023 71.3681 69.9654 67.2560 77.0856 66.9677 100.0000 0.0000 55.7452 71.0431 70.3357 67.3351 77.7512 67.0935 100.0000 0.0000 56.8594 71.6930 86.1967 86.1213 86.2721 31.3730 31.3005 31.4455 59.0677 58.7944 59.3409 73.9415 73.6511 74.2320
102.84 70.3555 67.2719 91.0635 67.2381 100.0000 -0.0000 56.4717 72.2996 70.1297 67.2350 90.6844 67.1791 100.0000 0.0000 55.9950 71.9722 70.5813 67.3088 91.4425 67.2971 100.0000 -0.0000 56.9485 72.6270 89.1162 89.0206 89.2118 30.3736 30.3020 30.4451 58.7186 58.4391 58.9981 76.8321 76.5779 77.0863
128.0 70.6625 67.1925 98.3942 67.0807 100.0000 -0.0000 55.9443 73.0737 70.4093 67.1525 98.2231 67.0012 100.0000 0.0000 55.4004 72.6581 70.9157 67.2326 98.5652 67.1603 100.0000 0.0000 56.4881 73.4892 90.4316 90.3459 90.5172 27.7893 27.7120 27.8665 63.8631 63.6271 64.0991 70.0363 69.7440 70.3285

==> data/scenario6.tex <==
param deepwalk dgi diffpool km mgcn2 mincut ortho sbm deepwalk_low dgi_low diffpool_low km_low mgcn2_low mincut_low ortho_low sbm_low deepwalk_high dgi_high diffpool_high km_high mgcn2_high mincut_high ortho_high sbm_high shchur shchur_low shchur_high agc agc_low agc_high sdcn sdcn_low sdcn_high daegc daegc_low daegc_high
4.0 66.4886 67.0601 56.0039 67.1102 99.7362 5.2085 56.5823 68.3377 66.3151 66.9906 55.7138 67.0464 99.6838 1.0724 56.1384 68.1317 66.6621 67.1297 56.2940 67.1739 99.7885 9.3446 57.0262 68.5437 74.8424 74.7769 74.9079 30.3216 30.2432 30.3999 39.2983 39.1075 39.4892 48.9171 48.6885 49.1456
5.0 66.7393 66.9770 54.6650 67.1056 99.6006 7.9576 56.0536 68.2815 66.5457 66.9162 54.3659 67.0378 99.5145 2.6684 55.5931 68.0848 66.9330 67.0378 54.9640 67.1734 99.6866 13.2468 56.5140 68.4782 74.5600 74.4928 74.6271 25.0867 25.0210 25.1523 34.6423 34.4579 34.8267 44.2619 44.1436 44.3802
7.0 66.3846 67.0230 50.9698 67.1679 99.6192 5.5307 55.5997 67.5406 66.1409 66.9493 50.6580 67.1144 99.5335 1.1886 55.2135 67.3632 66.6283 67.0967 51.2815 67.2215 99.7050 9.8727 55.9859 67.7181 73.5497 73.4808 73.6186 27.7159 27.6524 27.7794 37.7975 37.6216 37.9733 45.3643 45.1870 45.5415
9.0 66.0505 67.0363 48.4428 67.1223 99.4494 2.8102 55.8319 67.2986 65.7645 66.9504 48.1743 67.0510 99.3629 0.0447 55.3612 67.0467 66.3366 67.1221 48.7112 67.1937 99.5359 5.5757 56.3027 67.5505 72.9063 72.8296 72.9831 28.7213 28.6600 28.7826 37.2072 37.0223 37.3921 43.4846 43.3551 43.6142
12.0 65.9866 66.8604 46.1096 67.0982 98.3908 2.4069 55.4023 66.6642 65.6583 66.7683 45.8159 67.0356 97.7531 0.1905 54.9814 66.4340 66.3150 66.9525 46.4032 67.1608 99.0286 4.6234 55.8231 66.8944 71.6255 71.5514 71.6996 25.3366 25.2692 25.4040 36.2659 36.0995 36.4322 43.7894 43.6498 43.9290
17.0 65.7387 67.0309 42.9961 67.0846 97.8020 1.1454 55.1386 65.8014 65.3497 66.9319 42.6684 67.0207 96.9930 0.0000 54.7261 65.6000 66.1277 67.1299 43.3238 67.1485 98.6110 2.6962 55.5511 66.0028 69.3699 69.2982 69.4415 26.5677 26.5171 26.6182 34.5228 34.3394 34.7061 46.5455 46.4198 46.6713
23.0 65.6661 67.0847 40.6538 67.0591 97.0793 1.6745 54.7599 65.2799 65.2164 66.9883 40.3303 66.9947 96.1813 0.1252 54.3517 65.0261 66.1159 67.1811 40.9773 67.1236 97.9773 3.2238 55.1680 65.5338 66.8696 66.7950 66.9441 24.6390 24.5607 24.7172 33.3139 33.1537 33.4741 42.2832 42.1901 42.3764
30.0 64.9988 66.9808 38.7229 67.0647 96.0838 1.7272 54.8332 64.4190 64.5799 66.8331 38.3996 66.9911 95.1530 0.0000 54.3978 64.1680 65.4177 67.1285 39.0462 67.1383 97.0146 3.6427 55.2687 64.6699 64.7810 64.7025 64.8594 25.3253 25.2530 25.3976 32.2591 32.1170 32.4013 40.8040 40.6591 40.9490
41.0 64.1694 67.1658 37.6793 66.8836 93.0771 1.7569 54.3275 63.6185 63.6680 67.0026 37.3371 66.7849 91.4587 0.1751 53.9471 63.3308 64.6708 67.3290 38.0216 66.9824 94.6955 3.3387 54.7079 63.9061 60.6796 60.6063 60.7528 23.9460 23.8954 23.9966 31.7103 31.5768 31.8437 41.8475 41.7206 41.9745
55.0 63.7946 67.2128 36.8134 67.1519 89.1273 3.1820 55.1272 62.6143 63.2012 67.0703 36.4660 67.0925 87.3886 1.5692 54.6858 62.3049 64.3880 67.3553 37.1607 67.2113 90.8660 4.7947 55.5687 62.9237 60.0307 59.9668 60.0947 23.7257 23.6604 23.7910 30.8307 30.6931 30.9682 41.2857 41.1884 41.3830
74.0 61.6447 67.4019 35.6950 67.0899 88.2395 7.9183 54.3537 61.5539 61.1677 67.2663 35.4098 67.0193 86.9597 4.9129 53.9368 61.2058 62.1217 67.5375 35.9803 67.1605 89.5193 10.9238 54.7707 61.9020 58.7790 58.7185 58.8395 24.6438 24.5670 24.7206 30.8762 30.7331 31.0193 38.2425 38.1316 38.3533
99.0 61.6806 67.4532 36.0597 67.1565 85.1946 13.6889 54.5583 61.8316 61.1115 67.3156 35.6716 67.0921 83.2142 9.6353 54.1181 61.3130 62.2497 67.5908 36.4479 67.2209 87.1750 17.7426 54.9984 62.3502 57.8425 57.7780 57.9069 23.3002 23.2308 23.3697 30.2946 30.1593 30.4300 37.1198 37.0119 37.2276
132.0 59.3550 67.4623 35.4259 66.9812 78.2068 25.2929 53.5662 60.0349 58.7682 67.2992 35.1365 66.9101 76.0267 21.7799 53.2218 59.5741 59.9418 67.6253 35.7152 67.0523 80.3869 28.8060 53.9107 60.4958 55.0839 55.0296 55.1381 22.6168 22.5341 22.6995 28.0005 27.8630 28.1380 37.5832 37.4675 37.6989
177.0 59.0921 68.0217 35.5910 67.1048 81.8731 35.6604 53.7432 59.9180 58.5836 67.8778 35.2845 67.0399 80.0572 31.5914 53.3761 59.5654 59.6007 68.1655 35.8975 67.1698 83.6890 39.7294 54.1103 60.2706 54.7466 54.6908 54.8025 22.7801 22.7156 22.8447 28.9568 28.8172 29.0965 38.1268 38.0077 38.2458
237.0 57.7591 67.6438 35.1520 67.1294 74.0255 41.4408 53.7343 59.7250 57.1726 67.4232 34.8671 67.0531 71.7445 37.2854 53.2851 59.3037 58.3457 67.8644 35.4369 67.2058 76.3065 45.5962 54.1834 60.1464 54.0109 53.9602 54.0616 23.8618 23.7927 23.9310 30.2516 30.0940 30.4092 32.7831 32.6837 32.8825
318.0 55.7450 67.8946 35.3487 66.8962 74.7413 42.2817 53.2090 58.8957 55.1798 67.6862 35.1128 66.7916 72.3797 38.9026 52.8265 58.3345 56.3103 68.1031 35.5845 67.0008 77.1030 45.6608 53.5916 59.4569 52.0497 51.9790 52.1204 21.5789 21.4997 21.6581 26.4660 26.3347 26.5972 32.9115 32.7881 33.0348
426.0 55.2133 68.0761 35.2535 67.0662 78.2633 46.6678 52.8516 57.9655 54.6600 67.8947 35.0305 66.9951 76.2284 44.2119 52.4643 57.5689 55.7666 68.2575 35.4765 67.1373 80.2982 49.1238 53.2389 58.3622 52.0419 51.9887 52.0950 21.7881 21.7341 21.8421 25.2271 25.1023 25.3518 34.0358 33.9751 34.0965
571.0 52.1724 67.6173 35.7701 67.0563 75.4431 46.7121 52.6061 56.4170 51.4860 67.4309 35.5474 66.9793 73.3915 44.8015 52.2040 55.8871 52.8588 67.8038 35.9928 67.1332 77.4947 48.6227 53.0082 56.9470 50.5539 50.4891 50.6187 21.8369 21.7899 21.8840 25.0037 24.8750 25.1323 31.8273 31.7142 31.9404
764.0 49.6472 67.0129 35.7231 66.8927 72.6569 48.6549 51.3402 54.9792 48.8680 66.7978 35.3669 66.8066 70.4365 48.1033 50.9433 54.3833 50.4263 67.2281 36.0793 66.9789 74.8774 49.2064 51.7372 55.5752 50.5105 50.4484 50.5727 21.4787 21.4226 21.5348 25.4597 25.3499 25.5696 30.1164 29.9948 30.2380
1024.0 49.0557 68.0623 36.3258 67.1383 75.2235 46.2567 51.9799 54.4859 48.1654 67.8096 36.0538 67.0696 73.4979 44.6516 51.5620 53.8512 49.9460 68.3150 36.5979 67.2071 76.9490 47.8617 52.3978 55.1206 49.9495 49.8925 50.0065 22.2549 22.1879 22.3218 26.0806 25.9425 26.2187 27.8765 27.7836 27.9694
